Blockchain Based Decentralized Replay Attack Detection for Large Scale Power Systems

Large scale power systems are comprised of regional utilities with assets that stream sensor readings in real time. In order to detect cyberattacks, the globally acquired, real time sensor data needs to be analyzed in a centralized fashion. However, owing to operational constraints, such a centralized sharing mechanism turns out to be a major obstacle. In this paper, we propose a blockchain based decentralized framework for detecting coordinated replay attacks with full privacy of sensor data. We develop a Bayesian inference mechanism employing locally reported attack probabilities that is tailor made for a blockchain framework. We compare our framework to a traditional decentralized algorithm based on the broadcast gossip framework both theoretically as well as empirically. With the help of experiments on a private Ethereum blockchain, we show that our approach achieves good detection quality and significantly outperforms gossip driven approaches in terms of accuracy, timeliness and scalability.

==> junk.tex <==
%Consequently, there are only two choices that utility stakeholders are left with. One option (also the current industry practice) would be to rely solely on their local ICS detection mechanism to raise alarms. However, without the knowledge of a rapidly evolving state of global cyber health, the local mechanism will only raise an alarm when local assets are either i) under an attack themselves, or ii) are facing the system repercussions of a global attack on the network. In such circumstances, utilities would lose precious time which could otherwise be used to localize, diagnose and isolate faults. On the other hand, local detection schemes are inherently based on some underlying hypothesis test, which means that there is always some level of unavoidable false alarms. In large scale settings like the one considered in this paper, detection schemes could significantly overstate the cyber threat level since false alarm rates increase with the number of hypotheses tests being conducted \cite{benjamini2001control}. As a result, without active collaboration with other stakeholders, utilities might waste resources trying to diagnose false alarms unnecessarily.

%Therefore, there are only two possible paths that utility stakeholders can take. The first alternative (also the current industry practice) would be to rely solely on their local ICS detection mechanism to raise alarms. their own assets are either under attack or are facing the system disturbances due to a global attack on the network. Without being able to acquire a global view of cyber health in advance, utilities would lose precious time which could be used to localize, diagnose and isolate faults in order to counter the attack. The alternative is of course to continuously share local sensor data with a central repository and face a variety of technical, financial, legal, privacy and organizational challenges for the sole purpose of detecting global replay attacks. 

%While current state-of-the-art ICS attack detection methods are intended for individual plant sites and assets, this paper considers regional and global network attacks that require collaboration between the individual stakeholders. This collaborative setting involves ``pooling'' alarms from individual plants and assets, which tends to significantly reduce the false alarm rates. With current frameworks, such tasks, require competing stakeholders to share their data with a trusted third party which raises widespread privacy concerns. The U.S. Department of Energy operates the Cyber Risk Information Sharing Program (CRISP) \cite{multiYearPlan} which provides utility members with a platform specifically designed to share sensitive data. However, sharing data through a centralized repository presents several privacy risks along with efficiency and agility issues \cite{fisk2015privacy}. In the absence of legal obligation to participate, many critical utility providers do not pursue membership of data sharing cooperatives like CRISP. In addition, programs like CRISP also require hardware upgrades to existing IT infrastructure and associated costs as well \cite{multiYearPlan}. 

%A coordinated, ICS driven, replay attack that targets multiple utility based subsystems of the grid simultaneously would be poised to unleash a widespread outage \cite{rosas2007topological} on the entire grid.  Local disruptions at one utility could lead to widespread disruptions and cascading failures across sections of the grid  \cite{kinney2005modeling,bompard2011structural}. Such disruptions have been reported over the years \cite{venkatasubramanian2003analyzing}.  Diagnosis of cascading failures and their consequent localization and isolation becomes significantly difficult owing to the complex nature of the grid \cite{rosas2007topological}. On the other hand, current state-of-the-art ICS attack detection methods are intended only for individual plant sites and assets. As a result, existing frameworks for detecting globally coordinated attacks require competing stakeholders to share their low level sensor data itself with a trusted centralized repository. 

%Having discussed the nuances of global replay attack detection, we observe that the primary roadblock occurs because individual stakeholders must collaborate with each other to detect a global attack. Such a roadblock is inevitable despite the fact that stakeholders might be equipped with state of the art ICS attack detection mechanisms. Such mechanisms are only geared towards individual plant sites and assets and lack the ability to collaborate with others. 

%Therefore, there are only two possible paths that utility stakeholders can take. First path is to rely solely on their local ICS detection mechanism to raise alarms when their own assets are either under attack themselves or are facing the system disturbances due to a global attack on the network. Without being able to acquire a global view of cyber health in advance, utilities would lose precious time which could be used to localize, diagnose and isolate faults in order to counter the attack. The alternative is of course to continuously share local sensor data with a central repository and face a variety of technical, financial, legal, privacy and organizational challenges for the sole purpose of detecting global replay attacks. 




%In such circumstances, utilities would be \textit{flying blind} to the prospects of a large scale attack.

%Such collaborative setting requires ``pooling'' alarms from individual plants and assets, which tends to significantly reduce the false alarm rates. 

%Even though, current state-of-the-art ICS attack detection methods 
%are intended for individual plant sites and assets, this paper considers regional and global network attacks that require collaboration between the individual stakeholders.
%A decentralized mechanism allows individual plants and assets to leverage 

%While current state-of-the-art ICS attack detection methods are intended for individual plant sites and assets, this paper considers regional and global network attacks that require collaboration between the individual stakeholders.
%
%Owing to limitations arising from technical, legal, privacy and organizational aspects, a decentralized mechanism for globally coordinated replay attack detection becomes a lucrative alternative. 

%Why is a blockchain based mechanism needed?
%A mechanism is needed that preserves the privacy of data while extracting insights in a trustable fashion.
%Trust in the process peer to peer
%localization of data, eliminates the need to share raw sensor data.
%lowers the cost of the process
%setup cost is low
%instant insights

%have inherent distrust in federal programs pertaining to the
%Therefore, as a precursor for detecting a global attack, respective sensor information from all stakeholders must be available on a centralized repository. 

% There are data sharing programs which enable the sharing of real-time sensor level cyber incident data. For example, the U.S. Department of Energy operates the Cyber Risk Information Sharing Program (CRISP) \cite{multiYearPlan} which provides utility members with a platform specifically designed to share sensitive data. However, there are several limitations arising from a centralized paradigm as envisaged by CRISP. First, sharing data through a centralized repository presents several privacy risks \cite{fisk2015privacy,doe}. Moreover, there exists a lack of technical as well as legal provisions to prevent misuse of sensitive information contained in cyber incident reports. Second, without well established interoperable standards for data sharing, achieving consistency of data among the various participants is cumbersome. Third, centralized frameworks rely on a global aggregator which houses the data as well as performs periodic executions of the anomaly detection algorithm. Such a centralized global attack detection tactic might lead to issues in efficiency and agility \cite{fisk2015privacy}. Lastly, programs like CRISP require all the stakeholders to come to a mutual agreement regarding the financial, logistical and executive aspects of the centralized aggregator. 

%Permissioned blockchains provide the perfect decentralized computational platform for detecting global attacks. In our method, each stakeholder forms one node of a permissioned blockchain creating a global decentralized network. Blockchain based Smart Contracts (SC) provide a versatile computational platform for orchestrating business logic such as the global aggregation step in a purely decentralized fashion.  Owing to complete decentralized control the blockchain based solution ensures that benefits of a decentralized method remain intact while eliminating computational bottlenecks typically found in peer to peer decentralized algorithmic frameworks.


%Despite their benefits however, gossip protocols face several limitations especially in applications where locally reported states can change dynamically \cite{birman2007promise}. 





% A decentralized computational strategy helps eliminate data privacy concerns as well as infrastructure costs of a centralized paradigm. However, an information diffusion mechanism would also be required to determine the global state of cyber health based on locally reported alarm statistics. Gossip protocols are an important type of diffusion technique aimed at estimating the global state of a system in a peer-to-peer fashion \cite{boyd2006randomized,dimakis2006geographic,bg}. Among the state of the art gossip methods, Broadcast Gossip (BG) is considered to be a scalable, computationally efficient method that relies on neighbor based message exchanges in order to estimate the global state \cite{bg}. Despite their benefits however, gossip protocols face several limitations especially in applications where locally reported states can change dynamically \cite{birman2007promise}. 

% In this paper, we propose the use of the blockchain as a superior decentralization strategy for detecting globally coordinated replay attacks. Our decentralized framework ensures data privacy by allowing individual utilities to run their own detection algorithms locally. This leads to full data ownership with complete data privacy and eliminates the associated cost of setting up a trusted, centralized third party. Moreover, we utilize blockchain driven SmartContracts to estimate the likelihood of a global replay attack based on alarms and insights aggregated from the various utilities. From a computational standpoint, BG can be used for this purpose as well. Therefore, for benchmarking purposes, we also develop a BG based global replay attack detection detection framework for benchmarking purposes. We compare and contrast our blockchain driven approach against the BG in a theoretical as well as in an empirical manner. Our results indicate that the blockchain provides a sound computational platform allowing for global aggregation of local outputs in a timely, accurate and reliable fashion. The contributions of this work are summarized in detail below:

% We assume that plant dynamics can be modeled as a time-invariant linear system. Although this assumption is an oversimplification because physical plants are highly complex systems, it is needed to achieve a tractable and verifiable analytic framework that can serve as a foundation for future relaxations required to obtain more realistic models. Details of the regional detection model are discussed in subsection \ref{my:local}.

% In other words, the replay attack detection algorithms are executed locally at regional plant assets, whereas the global state of the entire network is assessed based on regional insights that are aggregated in a decentralized manner that preserves privacy. This model assumes that all regions are equally likely to experience a replay cyberattack and that attacks are mutually independent. Independence is assumed here for mathematical convenience. More importantly, a global network attack is assumed to occur when at least two regions report local attacks. 





%CRISP facilitates the gathering and analysis of cyber threat alerts in real time from all member utilities. 

%Limitations include the lack of interoperable standards, the absence of mechanisms to govern and control the use of sensitive information, and problems validating data quality. While centralized repositories, distribution lists and web services have been adopted in an attempt to address the requirement, the underlying needs are only partly met by these approaches, which do not deliver the required efficiency and effectiveness.

%data sharing argument
%then bring in why blockchain
%then contributions

%an important consequence of the high degree of interconnection is the distinct possibility of local events at the utility level disrupting operations at a global scale \cite{}.
%Many national power grids also incorporate a complex and diverse organizational structure comprising of numerous smaller subsystems\cite{}. For instance, the entire power infrastructure in continental United States can be categorized into deregulated or vertically integrated market environments. While the former delineates the role of production and transmission of power among different utilities \cite{}, the latter consists of a single organization in charge of both roles \cite{}. 

%the cyber risk associated with blah blah is exacerbated by 

With the integration of digital control and automation, national power grids are becoming increasingly vulnerable to cyber attacks in recent years \cite{ukraine}. In the absence of a global command centre, real time collection of global cyber health statistics becomes challenging on account of the diverse structural arrangement of the various participants.

%On account of structural diversities in power grids, 
%assessing the cyber health of the global power system becomes a challenge.

The national power grid of the United States is highly fragmented and has a mixed stake of ownership. In some parts of the country the grid operates as part of a deregulated market setup wherein multiple power utility companies come together to coordinate power supply. In other parts of the country, operations occur as part of a Vertically Integrated Market wherein one utility company commands production as well as supply. 

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.4\textwidth,keepaspectratio]{./images/pjm-zones2.pdf}
% %\includegraphics[height=6cm,trim=0cm 6cm 0cm 6cm,width=0.4\textwidth,keepaspectratio]{graphs/SweetSpotAnalysis.pdf}
% \caption{PJM RTO map along eastern United States\cite{PJM}}
% \label{fig:pjmzones} 
% \end{figure}

Figure \ref{fig:pjmzones} represents all the participating utility companies as part of the PJM Interconnect in northeastern United States. The sheer size and disparity of participating utility companies gives a glimpse of how complicated a power grid can be. Irrespective of market organization, a power grid can be thought of as a cluster of independent power regions which coordinate their operations with each other in a collective manner. In case of deregulated markets, this can be thought of as the various independent power utility companies whereas in case of vertically independent markets, these could be power subsidiaries of the parent company. 

 the power grid is becoming increasingly vulnerable to cyber attacks. However, a critical attack class is what is referred to as a multi-modal attack wherein multiple regions are attacked simultaneously. A primary instance of this was the cyber attack on Ukraine in 2015\cite{ukraine} wherein it took a while to recognize that a cyber attack had taken place.

\subsection{Detecting MultiModal Attacks: Why is it hard?}
The central point of contention is that every region might be managed by a different parent organization. In order to recognize that a global attack is taking place, local operators must first identify that failures taking place locally are indeed the result of a cyber attack.

A malicious attacker might start orchestrating a multi modal attack in order to cause widespread outage. Therefore, there must be a technique for all regions to monitor the global health of the system in a decentralized manner continuously. Unfortunately this is not the case due to various operational, logistical organizational and political reasons.  
\begin{itemize}
\item In case of mixed market organizational structure like in North America, where there is a combination of deregulated and vertically integrated markets, setting up of a central command centre for monitoring the national power grid in real time is expensive and requires legislative will.
\item In the continental United States, there is no legislative requirement that enforces sharing of real time diagnostic information for monitoring global cyber health of the power grid\cite{esiac}.
\item Utility companies are wary of sharing real time sensor data with their peers. In addition, sharing of data requires specialized network, hardware and software support that increases operating costs of the utility companies.
\item Further utility companies do not want to share their local infrastructural information pertaining to asset ownership, operational characteristics and local consumer demand and supply profiles\cite{fakebc,bc_intrusion}. Additionally, privacy of infrastructure data would be an important consideration in the future as we head towards Smart Cities \cite{privacy}.
\item Further, federal efforts like the CRISP program \cite{CRISP} of the Department of Energy are voluntary initiatives which do not encompass all the utility companies.
As a result only 75\% of end consumers are covered by CRISP, leaving a significant 25\% of national consumers without any protection from cyber attacks\cite{CRISP}. 
\item For programs like CRISP, participating utilities incur significant overhead pertaining to additional hardware installations, augmenting existing corporate firewalls and annual subscription fees for participation in the program. 

Such constraints make it cumbersome for utilities to participate and pose as a significant stumbling block for achieving 100\%  consumer coverage from cyber attacks.   

\end{itemize}

\subsection{SmartContracts : Blockchain for Cybersecurity of the Grid}
Therefore, in order to thwart such a multi modal attack information sharing is essential in order to detect the global system state with due cognizance of the challenges mentioned above.

Smart Contracts offer a viable alternative to solve this problem because:
\begin{itemize}
    \item They offer a capability to keep track of global system state in a completely decentralized manner.
    \item They can be designed in such a way that local infrastructural data is kept local to each region and only a distress signal value can be shared.
    \item They can be readily implemented on a private blockchain like Ethereum and require only access to the internet. This implies that utilities have a significant reduction of costs in their efforts to detect a global attack.
\end{itemize}

\subsection{Contribution}
\begin{itemize}
\item We utilize a local algorithm which can detect a local attack based on streaming sensor data collected at the regional level. The objective of this paper is to scale it to a large scale network and determine a global attack in a decentralized manner. Therefore, it is assumed that each region is reporting a diagnostic alarm message based on its local reading. This forms the data that is sent to the smart contract to be evaluated. We perform bayesian inference on the data reported by all regions to determine the global system state.

\item A smart contract is not a very computational efficient mechanism to compute the global state. Therefore, an expensive operation like a bayesian inference needs to be done in a very computationally efficient manner. We derive a theorem specifically for use on a smart contract Decentralized Application(DAPP).

\item The Theorem only comprises of a global sum and one multiplication operation that needs to be computed based on latest available values to the smart contract. 

\item Experimental results on an actual power system test case using a smart contract developed using Solidity on a private Ethereum network is demonstrated.
\end{itemize}
